A method for Selecting Scenes and Emotion-based Descriptions for a Robot's Diary

In this study, we examined scene selection methods and emotion-based descriptions for a robot's daily diary. We proposed a scene selection method and an emotion description method that take into account semantic and affective information, and created several types of diaries. Experiments were conducted to examine the change in sentiment values and preference of each diary, and it was found that the robot's feelings and impressions changed more from date to date when scenes were selected using the affective captions. Furthermore, we found that the robot's emotion generally improves the preference of the robot's diary regardless of the scene it describes. However, presenting negative or mixed emotions at once may decrease the preference of the diary or reduce the robot's robot-likeness, and thus the method of presenting emotions still needs further investigation.

==> src/acknowledge.tex <==
\section*{ACKNOWLEDGMENT}

The preferred spelling of the word acknowledgment in America is without an e after the g. Avoid the stilted expression, One of us (R. B. G.) thanks ...  Instead, try R. B. G. thanks. Put sponsor acknowledgments in the unnumbered footnote on the first page.

References are important to the reader; therefore, each citation must be complete and correct. If at all possible, references should be commonly available publications.


